Full Transport General Relativistic Radiation Magnetohydrodynamics for Nucleosynthesis in Collapsars

We model a compact black hole-accretion disk system in the collapsar scenario with full transport, frequency dependent, general relativistic radiation magnetohydrodynamics. We examine whether or not winds from a collapsar disk can undergo rapid neutron capture (r-process) nucleosynthesis and significantly contribute to solar r-process abundances. We find the inclusion of accurate transport has significant effects on outflows, raising the electron fraction above $Y_{\rm e} \sim 0.3$ and preventing third peak r-process material from being synthesized. We analyze the time-evolution of neutrino processes and electron fraction in the disk and present a simple one-dimensional model for the vertical structure that emerges. We compare our simulation to semi-analytic expectations and argue that accurate neutrino transport and realistic initial and boundary conditions are required to capture the dynamics and nucleosynthetic outcome of a collapsar.

==> Makefile <==
LATEXMK=latexmk

SRC=header.tex \
    nubhlight.bib

all: collapsar.pdf

collapsar.pdf: collapsar.tex ${SRC} $(shell find figures/)
	${LATEXMK} -f -pdf $<xb

clean:
	rm -f ./*.aux ./*.bbl ./*.blg ./*.log ./*.nav ./*.out ./*.snm ./*.toc ./*.fls ./*.fdb_latexmk collapsarNotes.bib collapsar.pdf *.synctex.gz auto


